Generalization in Transfer Learning

Agents trained with deep reinforcement learning algorithms are capable of performing highly complex tasks including locomotion in continuous environments. We investigate transferring the learning acquired in one task to a set of previously unseen tasks. Generalization and overfitting in deep reinforcement learning are not commonly addressed in current transfer learning research. Conducting a comparative analysis without an intermediate regularization step results in underperforming benchmarks and inaccurate algorithm comparisons due to rudimentary assessments. In this study, we propose regularization techniques in deep reinforcement learning for continuous control through the application of sample elimination, early stopping and maximum entropy regularized adversarial learning. First, the importance of the inclusion of training iteration number to the hyperparameters in deep transfer reinforcement learning will be discussed. Because source task performance is not indicative of the generalization capacity of the algorithm, we start by acknowledging the training iteration number as a hyperparameter. In line with this, we introduce an additional step of resorting to earlier snapshots of policy parameters to prevent overfitting to the source task. Then, to generate robust policies, we discard the samples that lead to overfitting via a method we call strict clipping. Furthermore, we increase the generalization capacity in widely used transfer learning benchmarks by using maximum entropy regularization, different critic methods, and curriculum learning in an adversarial setup. Subsequently, we propose maximum entropy adversarial reinforcement learning to increase the domain randomization. Finally, we evaluate the robustness of these methods on simulated robots in target environments where the morphology of the robot, gravity, and tangential friction coefficient of the environment are altered.

==> files/coverletter.tex <==
Dear Editor-in-Chief of Robotics and Autonomous Systems,

We would like to submit our manuscript titled "Generalization in Transfer Learning" by S. E. Ada, E. Ugur, and H. L. Akin.  In this work, we propose a set of methods and regularization techniques for deep reinforcement learning in the transfer learning domain. There has been an increasing interest in using policy gradient algorithms and adversarial reinforcement learning methods in transfer reinforcement learning. Using a humanoid and a hopper robot, we evaluate our methods in 18 different settings in inter-robot bipedal locomotion, morphology transfer, and environment domain shift in gravity and friction cases.

Our methods can extract generalizable skills from a single source task that can be transferred to a variety of target tasks. In doing so, we hope robots in the future will not need additional training in every domain shift and resort to prior knowledge. Inspired by real-life use cases we designed the following target tasks: a taller and heavier humanoid, a shorter and lighter humanoid, a delivery humanoid. For instance, without having any knowledge of carrying extra weight, the delivery humanoid robot is required to carry a heavy box in one hand. Furthermore, we adjusted gravity and friction in the target tasks to demonstrate transfer in different planets and surfaces. To show adversarial RL algorithms are enhanced using our methods compared to the baselines, we change the mass of the torso of a Hopper robot and the gravity of the environment. 

We increase the generalization capacity of one of the widely used policy gradient algorithm named Proximal Policy Optimization (PPO) by using a set of regularization techniques. The performance of a policy in the source task does not provide an insight into the performance in the target task. In accordance, we address the problem of overfitting in deep transfer RL. Previous works on transfer deep reinforcement learning do not apply regularization before benchmarking which results in inaccurate comparisons of methods. We show that regularized PPO can be transferred to a wider range of continuous control tasks than Robust Adversarial Reinforcement Learning (RARL). We propose a novel way of utilizing critic networks, and maximum entropy in RARL that improves performance in the target task. 

We believe that our contributions to the areas of  "Transfer Learning",  "Generalization in Deep Reinforcement Learning", "Robot Locomotion", in this manuscript will be of interest to the readers of Robotics and Autonomous Systems. 

Thank you for your consideration of this manuscript.

Sincerely yours, 
Suzan Ece Ada, MSc.
Ph.D. student, Computer Engineering, Bogazici University
